Shirakami: A Hybrid Concurrency Control Protocol for Tsurugi Relational Database System

Bill-of-materials and telecommunications billing applications need to process both short and long read-write transactions simultaneously. Recent work rarely addresses such evolving workloads. To deal with these workloads, we propose a new concurrency control protocol, Shirakami. Shirakami is a hybrid protocol. The first protocol, Shirakami-LTX, is for long read-write transactions based on multiversion view serializability. The second protocol, Shirakami-OCC, is for short transactions based on Silo. Shirakami naturally integrates them with write-preservation and epoch-based synchronization. It does not require dynamic protocol switching and provides stable performance. We implemented Shirakami as the transaction processing module of the Tsurugi system, which is a production-grade relational database system. The experimental results demonstrated that Tsurugi was at least 7.9x faster than PostgreSQL, and Shirakami-LTX exhibited 680x higher throughput than Shirakami-OCC.

==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> alg-ltx_old.tex <==
\begin{algorithm}[tb]
\caption{Shirakami-LTX Protocol}
\label{alg:shirakami-ltx}
\DontPrintSemicolon
\small
\Input{A transaction $tx$}
\Output{COMMIT or ABORT}

\tcp{Entry Point}
\If{$tx.type = \text{LTX}$}{
    \Return \FExecLTX{$tx$}\;
}
\ElseIf{$tx.type = \text{OCC}$}{
    \Return \FExecOCC{$tx$}\;
}

\BlankLine

\SetKwBlock{FnLTX}{function \FExecLTX{$tx$}}{end}
\FnLTX{
    $tx\_id \gets \text{assign\_transaction\_id}()$\;
    $commit\_epoch \gets \text{get\_global\_epoch}() + 1$\;
    $\text{register\_wp}(tx.wp\_set, tx\_id, commit\_epoch)$\;
    
    \tcp{Execution Phase}
    $overtaken\_set \gets \emptyset, max\_read\_epoch \gets 0, read\_set \gets \emptyset, write\_set \gets \emptyset$\;
    \ForEach{$opr \in tx$}{
        \eIf{$opr.type = \text{READ}$}{
            $overtaken\_set \gets overtaken\_set \cup \{id \in \text{WP}(opr.key) : id < tx\_id\}$\;
            $value, ver \gets \text{read\_snapshot}(opr.key, commit\_epoch)$\;
            $read\_set \gets read\_set \cup \{opr.key\}$\;
            $max\_read\_epoch \gets \max(max\_read\_epoch, ver.epoch)$\;
        }{
            $write\_set \gets write\_set \cup \{opr\}$\;
        }
    }
    
    \tcp{Order Forwarding}
    \ForEach{$ltx\_id \in overtaken\_set$}{
        $\text{wait\_for\_completion}(ltx\_id)$\;
        \If{$\text{committed}(ltx\_id) \land (read\_set \cap \text{write\_keys}(ltx\_id) \ne \emptyset)$}{
            $new\_epoch \gets \min(commit\_epoch, \text{commit\_epoch\_of}(ltx\_id))$\;
            \tcp{Read Validation}
            \If{$max\_read\_epoch \ge new\_epoch$}{ \Return{ABORT} }
            $commit\_epoch \gets new\_epoch$\;
        }
    }
    
    \tcp{Write Validation}
    \ForEach{$opr \in write\_set$}{
        \If{$commit\_epoch \le \text{max\_reader\_epoch}(opr.key)$}{ \Return{ABORT} }
    }
    
    $\text{register\_reader\_epoch}(read\_set, commit\_epoch)$\;
    $\text{apply\_writes}(write\_set, commit\_epoch)$\;
    \Return{COMMIT}\;
}
\end{algorithm}


==> author.tex <==
\author{%
\alignauthor
\IEEEauthorblockN{Takashi Kambayashi}\\
\IEEEauthorblockA{NAUTILUS Technologies, Inc}
\and
\IEEEauthorblockN{Takayuki Tanabe}\\
\IEEEauthorblockA{NAUTILUS Technologies, Inc}
%Tokyo\\
%tanabe@nautilus-technologies.com}
\and
\IEEEauthorblockN{Takashi Hoshino}\\
\IEEEauthorblockA{Cybozu Labs}
%Tokyo\\
%hoshino@labs.cybozu.co.jp}
\and
\IEEEauthorblockN{Hideyuki Kawashima}\\
\IEEEauthorblockA{Keio University}
%Fujisawa\\
%river@sfc.keio.ac.jp}
}

\if 0
\numberofauthors{1} 
\author{
\alignauthor
Takashi Kambayashi$^1$,
Takayuki Tanabe$^2$,
Takashi Hoshino$^3$,
Hideyuki Kawashima$^4$
\affaddr{$^{1,2}$NAUTILUS Technologies, Inc., $^3$Cybozu Labs, Inc., $^4$Keio University}\\
%\email{tanabe@nautilus-technologies.com, hoshino@labs.cybozu.co.jp,\\river@sfc.keio.ac.jp, tatebe@cs.tsukuba.ac.jp}
\affaddr{$^1$kambayashi@nautilus-technologies.com, $^2$tanabe@nautilus-technologies.com, $^3$hoshino@labs.cybozu.co.jp,$^4$river@sfc.keio.ac.jp}
}


\numberofauthors{4} 
\author{
% 1st. author
\alignauthor
Takayuki Tanabe\titlenote{Work done while at University of Tsukuba}\\
       \affaddr{NAUTILUS Technologies, Inc}\\
       \email{tanabe@nautilus-technologies.com}
% 2nd. author
\alignauthor
Takashi Hoshino\\
       \affaddr{Cybozu Labs}\\
       \email{hoshino@labs.cybozu.co.jp}
% 3rd. author
\alignauthor
Hideyuki Kawashima\\
       \affaddr{Keio University}\\
       \email{river@sfc.keio.ac.jp}
\and  % use '\and' if you need 'another row' of author names
% 4th. author
\alignauthor
Osamu Tatebe\\
       \affaddr{University of Tsukuba}\\
       \email{tatebe@cs.tsukuba.ac.jp}
}
\fi


==> header.tex <==
\usepackage{graphicx}
\usepackage{balance}  % for  \balance command ON LAST PAGE  (only there!)
\usepackage{caption}
\usepackage{subcaption}
\usepackage{ascmac}
\usepackage{multirow}
\usepackage{seqsplit}
% It should be used on writing.
\usepackage{color}
% It is required to use \url in bibliography for arXiv.
\usepackage{url}
\usepackage{cite}

% make caption info bold
\makeatletter
\long\def\@makecaption#1#2{% \@makecaption を再定義します
\vskip\abovecaptionskip
\iftdir\sbox\@tempboxa{#1\hskip1zw#2}%
\else\sbox\@tempboxa{\textbf{#1:} #2} % ここを変更する
\fi
\ifdim \wd\@tempboxa >\hsize%
\iftdir #1\hskip1zw#2\relax\par
\else \textbf{#1:} #2\relax\par\fi% ここを変更する
\else
\global \@minipagefalse
\hbox to\hsize{\hfil\box\@tempboxa\hfil}
\fi
\vskip\belowcaptionskip}
\makeatother


\hyphenation{CC-Bench}

% Include information below and uncomment for camera ready

\ifvldb
\vldbTitle{An Analysis of Concurrency Control Protocols for In-Memory Databases with CCBench}
\vldbAuthors{Takayuki Tanabe, Takashi Hoshino, Hideyuki Kawashima, Osamu Tatebe}
%\vldbDOI{https://doi.org/10.14778/xxxxxxx.xxxxxxx}
\vldbDOI{https://doi.org/10.14778/3424573.3424575}
\vldbVolume{13}
\vldbNumber{13}
\vldbYear{2020}
\else
%\title{An Analysis of Concurrency Control Protocols for In-Memory Database with CCBench.}
%\authors{Takayuki Tanabe, Takashi Hoshino, Hideyuki Kawashima, Osamu Tatebe.}
%\DOI{https://doi.org/10.14778/xxxxxxx.xxxxxxx}
%\Volume{13}
%\Number{46}
%\Year{2020}
\fi

\begin{document}
\input{title}
\input{author}


==> proposal-kam.tex <==
\section{提案：Shirakami}
\subsection{短期TX用CC}
\subsection{長期TX用CC}
\begin{itemize}
 \item epoch based snapshot read

 開始時点でのTSでの最新のデータセットを読む。通常のMVTOと同じ。ただし、各epochで投入するLTXの読むべきデータセットはepoch投入時に確定している。これにより、同じepochで始まるLTXが別々のversionを読むことがなくなり、複数のversionが読まれることによるcontentionを低減することができる。デメリットとしては、データが1epoch分staleになる。しかし、最新のversionを読むのであればOCCで読めば良いし、LTXではabort率の低減が最大の目標であるので、メリットの方が大きい

 \item order forwarding

conflictを解決するために後続順序のtransactionの前置ができる。通常のMVTOでは前置せずにabortする。MVTOよりも強いserialization powerを獲得している。

 \item two-sided validation

order forwardingをしつつ、serializableを確保する必要がある。そのために、read/write それぞれのconflictを検出し、serializableでない場合はabortする。LTXでは、自分のover-writerが存在するとき（read conflict）、自分の前置ができる範囲で自分のwriteが他のtransactionのreadを阻害する場合(write conflict)はabortする。

 \item read conflict

 \begin{itemize}
  \item 自分よりも先に開始しているTxで、自分の開始時点には未コミットなtransactionについて
	
	自分が読んでいるversionに上書きし、新たなversionを加える場合
	
  \item 自分の開始時点ではすでに完了しているtransactionについて
	
	　自分が読んでいるversionが、そのtransactionに上書きされている場合
	に発生する
	このとき、自分のserialization orderを、read conflictを起こしているtransactionのserialization orderよりも前置できれば、自分のread fromを保護することができる。
 \end{itemize} 
 
 \item write conflict
 
 read conflictを解消するために、前置した時に、自分のtransactionのwriteが、自分よりも後置されるtransactionのreadを阻害する場合はwrite conflictが発生してabortになる
 
 read conflictとwrite conflictの両者のconflictが成立したとき、その時に限りabortになる（2-sided validation）
 MVTOではread conflictだけabortになるが、shirakamiはそこから、order forwardingを試み、失敗した場合のみabortとしている
 
 \item boundary
 
 order forwardingを試みる際に、トランザクション間でcascadingが発生する。このときの最後置されるtransactionの開始timestampをboundaryとよび、cascadingするtransaction間でpropagateさせる。このboundary以降でのreadについてtransactionはwrite conflictを判定する。
 
 \item read protocol
 
 各transactionが複数のreadを行うとき、そのreadするversionをwriteしているtransactionのboundaryの集合の最小値をread upper boundと呼ぶ。read upper boundが自分のboundaryを越えた場合は read skewが発生するのでabortとなる
 
 \item waiting processing
 
 OCCは短いトランザクションを想定しているため、validationはシビアではなく、大きな偽陽性を許容している。これに対してLTXは長いトランザクションを想定しており、OCCがabort  and retryによるトランザクションの実行可能性を上げているのに対して、LTXはabortコストが高く、可能な限り偽陽性を減らす必要がある。

問題になるのは、自分よりも優先度の高いトランザクションについて、自分と競合する可能性があるときに、そのトランザクションの結果を待たないと自身のcommit/abortが決定できない場合であり、この場合LTXでは各epochの切れ目ごとに、その決定可能性をwaitすることができる。また、あまりにwaitが長い場合は、ユーザサイドでepochの切れ目ごとにabort指示を介入させることも可能である。

このwaitには2種類存在し、両者ともにwaiting listで管理される。lock制御とことなり、waitする先は必ず自分よりも優先度高いトランザクションになるため、dead lockは発生しない

 \item boundary wait

 boundaryが確定するのは
1.自分のread operationが終わっていること
2. そのread operationのoverwriteのtxのread operationが終わっていること
1-2を再帰的に完了したときに確定する。すなわち自分がpre-commit状態になってもboundaryは確定しない　
自分のboundaryを確定させるために、自分のreadのover writerがcommitしていない場合は、そのover writerがcommitまたはabortされるまで待つ。なお、自分がwaited byの場合は、自分がcommit/abort時点で処理を
する。

 \item read wait

 自分のoperationにwriteが確定しているときで、readはすべて完了して、precommit状態である場合に、

自分以前に開始しているTxで
1：boundaryが自分と同じか、自分よりも後のTxで
2：自分がwriteするpageのreadがないとき（write conflictがいまだ発生していない場合、発生している場合はこの時点でabortされる）
3：write conflictが発生する可能性があるため、該当Txが終了するまで、waitする
これはそもそもover writerが存在していない場合は不要である。


 \item read restriction

 Waitingのワークアラウンドとして、ユーザ側でそもそもread“しない”page setを指定して、conflictを回避するメカニズムを提供する。これはたとえばread and reportのように、長いトランザクションが走っている最中に、そのトランザクションがwriteするtableにアクセスし、更新前のversionを集計するような場合では極めて有効である。

 \item priority control

 一般にlock処理は、serialization orderの確保の目的で導入されるが、RDB上での実践的な用途はtransactionの優先制御に利用されている。すなわち競合する可能性が高いtransactionを同時に実行する場合、より優先度の高いtransactionに先にlockをかけて保護する。したがって、楽観処理のCCでlockに代わるメカニズムを導入しないかぎり、各トランザクションの優先制御を行うことができない。

 LTXでは、以下の仕組みを導入することにより、lockではない優先度管理を行っている
 ・LTX間では開始TSが小さい方が優先される
 ・OCC間では優先度管理は行わない
 ・すべてのLTXはすべてのOCCに優先する
\end{itemize}





\subsection{長期と短期を同時に扱う手法}
LTXはserialization powerが強く、代償としてオーバーヘッドが大きい。一方OCCはserialization powerが弱いが、そのメリットとしてオーバーヘッドが小さい。比較的小さく細かいトランザクションはretryコストが低いため、serialization powerが弱いことによるabort率の増大もretryを行うことでカバーアップできるため、OCCで行うことが全体のスループットを上げることができる。その一方で大きな粒度のトランザクションはretryコストが高く、serialization powerが弱いことによるabort率の増大は大きなデメリットがあり、多少のオーバーヘッドがあってもserialization powerを上げてabort率を低減させた方が全体のスループットは上がる。すなわち小さい短いトランザクションはOCCで、大きな長いトランザクションはLTXで、と選択的にCCを利用して、両者が同時に処理できるようにすると全体のスループットはあがる

これを達成するには、OCCはそれ単独ではserializableであり、またLTXもそれ単独ではserializableである、ことを踏まえ、その上で両者の順序を合成したときにserializableである必要がある

\subsubsection{OCCとLTXのcombinedの処理}

Epoch based Concurrency Controlを行う。よって
・epoch開始時点
-継続しているOCCとLTX
-このepochで開始されるLTX
-このepochで開始されるOCC
の3種類のTxが開始時点に存在する

LTXは開始時点でread対象となるread setをそのepochで指定される。SQLレイヤーから投入されたLTXは各epochではまずqueueingされ、次の開始epochにread対象が明確にalignされた段階で、epochの開始時点にまとめて順次投入される。このとき、LTXは開始のbegin timestampで順序付けされる。

また、OCCがepoch単位でread alignされる必要がないので、epochの最中に順次投入され、epoch終了時点でcommit readyになっているものがvalidationされorderが決定される。このとき、OCCは終了時のcommit timestampで順序付けされる。

したがって、各epochでのserialization orderは、必ず[LTX*]<[OCC*]になっている。LTX内部/OCC内部ではすべて順序はとれているので、各LTXとOCCで順序がとれないときに、LTXとOCCではLTXが優先されるために、OCCはabortされなくてはならない。

\subsubsection{wrte preserve}
LTXがOCCと共存し、LTXがOCCに優先するために、LTXでは書き込みを行うPageまたはPage set（現在の実装はPage set）に対してTx開始時点に明示的に宣言を行う。これをwrite preserveと呼ぶ。これによりWPを行ったLTXよりも後で開始されるconcurrentなすべてのTxは、自分よりも優先度の高いLTXのwriteを知ることができるため、自分の優先度が低い場合は自分でabortすることができる。なお、LTXは自分のcommit時点で自分の宣言したWPとは異なるwriteをした場合はabortされる

\subsubsection{read only transaction}
最新のversionだけで構成されたデータセットを読む場合、over-writerが存在する場合は常にread skewが発生する可能性があり、abort riskがある。この場合、たとえばSQLから見た場合は、単純なSELECT文がabortされることになり、従来のユーザの直感に反する。

Tsurugiでは以下の方法によりread only transactionを保護し、正当なデータセットを読めるようにしている

OCCではパフォーマンスを優先したabort and retryなのでread onlyとread and writeでは区別はしない。常に最新のversionを読みたい場合にOCCで選択的にtransactionを投入する。たとえば上記の例でいえば、(x0,y1,z2)のデータセットを読むチャンスは与えられなければならない（ただし、この時に同時にa0を読む場合はabortされる）このようなケースではOCCを利用する

これに対してLTXはユーザに選択的に2種類のSnapshotを読むことを許可する。一つはSafeであり、もう一つはUnsafeである。

\subsection{safe snapshot}
Tsurugiでは各epochの終わりに毎回かならず最新のsnapshotが作れる。このときそのsnapshotを構成するversion対してover writerが存在しない場合に、それをsafe snapshotとし、そうでない場合unsafe snapshotとする。Safe を読んだ場合は read skewは発生しない

SSのboundary=0とする。ROのboundaryはoverwriterが発生しないので、beginTS=1とすると　RO.boundaryは常に1でRUB＝0より　常にRUB＜RO.boundary

TsurugiではROであれば、常にSafeを読む。read and writeの場合は指定しない場合はunsafeを読む。（ROでunsafeを読みたい場合はOCCで起動する）

\begin{itemize}
 \item running exampleを入れたい
\end{itemize}

==> title.tex <==
%\title{Shirakami: A Modern Hybrid Concurrency Control Protocol for New Generation RDB ``Tsurugi''}

%\title{Shirakami: A Novel Effective Hybrid Concurrency Control Protocol for Lightening Speed RDB ``Tsurugi''}

\title{Shirakami: A Hybrid Concurrency Control Protocol for Tsurugi Relational Database System}

